Magnetic Field Sensing for Pedestrian and Robot Indoor Positioning

In this paper we address the problem of indoor localization using magnetic field data in two setups, when data is collected by (i) human-held mobile phone and (ii) by localization robots that perturb magnetic data with their own electromagnetic field. For the first setup, we revise the state of the art approaches and propose a novel extended pipeline to benefit from the presence of magnetic anomalies in indoor environment created by different ferromagnetic objects. We capture changes of the Earth's magnetic field due to indoor magnetic anomalies and transform them in multi-variate times series. We then convert temporal patterns into visual ones. We use methods of Recurrence Plots, Gramian Angular Fields and Markov Transition Fields to represent magnetic field time series as image sequences. We regress the continuous values of user position in a deep neural network that combines convolutional and recurrent layers. For the second setup, we analyze how magnetic field data get perturbed by robots' electromagnetic field. We add an alignment step to the main pipeline, in order to compensate the mismatch between train and test sets obtained by different robots. We test our methods on two public (MagPie and IPIN'20) and one proprietary (Hyundai department store) datasets. We report evaluation results and show that our methods outperform the state of the art methods by a large margin.

==> tables/Tables/classification_results.tex <==
\begin{table}[h!]
\centering

\begin{tabular}{ |c|c|c| }
\hline
\textbf{Building} & \textbf{Accuracy (\%)} \\ \hline
CSL & 95.60 \\ \hline
Loomis & 81.06 \\ \hline
Talbot & 72.41  \\ \hline

\end{tabular}
\caption{Classification model results}
\label{tab:class_results}
\end{table}

==> tables/Tables/csl_regr_full_results.tex <==
%\newgeometry{margin=1cm} % modify this if you need even more space
\begin{landscape}

\begin{table}[h!]
\centering

\begin{tabular}{ |c|c|c|c|c|c|c| }
\hline
\textbf{Test error (m.)} & \textbf{dropout} & \textbf{image\_size} &  \textbf{loss} &
 \textbf{metrics} &
 \textbf{mag\_comp} &
 \textbf{window}
 \\ \hline
0.5833 & 0.3 & 24 & mae & canberra & xyz & 10.0 \\ \hline
0.6011 & 0.5 & 36 & huber & jaccard & xyz & 10.0 \\ \hline
0.6051 & 0.7 & 36 & mae & canberra & xyz & 10.0 \\ \hline
0.628 & 0.7 & 36 & mae & canberra & xyz & 10.0 \\ \hline
0.6346 & 0.5 & 36 & huber & canberra & xyz & 10.0 \\ \hline
0.6382 & 0.5 & 36 & huber & canberra & xyz & 7.0 \\ \hline
0.6711 & 0.5 & 36 & huber & euclidean & xyz & 10.0 \\ \hline
0.6738 & 0.3 & 36 & huber & canberra & xyz & 7.0 \\ \hline
0.6821 & 0.5 & 36 & huber & minkowski & xyz & 10.0 \\ \hline
0.7168 & 0.3 & 24 & mae & canberra & xyz & 10.0 \\ \hline
0.7272 & 0.7 & 36 & mae & jaccard & xyz & 10.0 \\ \hline
0.734 & 0.7 & 36 & huber & canberra & z\_xy\_xyz & 10.0 \\ \hline
0.7348 & 0.3 & 36 & mae & minkowski & xyz & 10.0 \\ \hline
0.7611 & 0.3 & 36 & huber & canberra & xyz & 10.0 \\ \hline
0.7647 & 0.7 & 36 & mae & minkowski & xyz & 10.0 \\ \hline
0.7734 & 0.7 & 36 & huber & minkowski & xyz & 10.0 \\ \hline
0.7751 & 0.3 & 36 & mae & euclidean & xyz & 10.0 \\ \hline
0.7792 & 0.3 & 36 & mae & euclidean & z\_xy\_xyz & 10.0 \\ \hline
0.7871 & 0.5 & 36 & mae & jaccard & xyz & 10.0 \\ \hline
0.7903 & 0.3 & 36 & mae & jaccard & xyz & 10.0 \\ \hline
0.7983 & 0.5 & 36 & mae & jaccard & xyz & 10.0 \\ \hline
0.8 & 0.3 & 36 & mae & minkowski & xyz & 7.0 \\ \hline
0.8001 & 0.7 & 36 & mae & euclidean & z\_xy\_xyz & 10.0 \\ \hline
0.8002 & 0.3 & 36 & mae & canberra & xyz & 10.0 \\ \hline
0.8198 & 0.5 & 36 & mae & euclidean & xyz & 10.0 \\ \hline
0.8208 & 0.5 & 36 & mae & minkowski & z\_xy\_xyz & 10.0 \\ \hline
0.8281 & 0.5 & 36 & mae & minkowski & xyz & 10.0 \\ \hline
0.8297 & 0.5 & 36 & mae & euclidean & xyz & 7.0 \\ \hline
0.8348 & 0.5 & 24 & huber & euclidean & xyz & 10.0 \\ \hline
0.8418 & 0.5 & 36 & mae & canberra & z\_xy\_xyz & 10.0 \\ \hline
0.8478 & 0.5 & 36 & mae & minkowski & z\_xy\_xyz & 10.0 \\ \hline
0.8481 & 0.7 & 36 & mae & minkowski & xyz & 10.0 \\ \hline
0.849 & 0.5 & 24 & mae & canberra & xyz & 10.0 \\ \hline
0.8506 & 0.7 & 36 & mae & minkowski & xyz & 10.0 \\ \hline
0.8558 & 0.7 & 36 & mae & canberra & z\_xy\_xyz & 10.0 \\ \hline
0.8587 & 0.3 & 36 & huber & canberra & xyz & 7.0 \\ \hline
0.8621 & 0.7 & 36 & huber & canberra & xyz & 7.0 \\ \hline
0.8653 & 0.7 & 36 & mae & euclidean & z\_xy\_xyz & 10.0 \\ \hline
% 0.8655 & 0.5 & 36 & mae & euclidean & xyz & 10.0 \\ \hline
% 0.8693 & 0.3 & 36 & mae & canberra & xyz & 10.0 \\ \hline
% 0.8714 & 0.3 & 24 & mae & jaccard & xyz & 10.0 \\ \hline
% 0.8907 & 0.5 & 36 & huber & euclidean & z_xy_xyz & 10.0 \\ \hline
% 0.8911 & 0.5 & 36 & huber & canberra & z_xy_xyz & 10.0 \\ \hline
% 0.8916 & 0.5 & 24 & huber & minkowski & xyz & 10.0 \\ \hline
% 0.9002 & 0.5 & 36 & mse & canberra & xyz & 10.0 \\ \hline
% 0.9026 & 0.7 & 36 & huber & euclidean & z_xy_xyz & 10.0 \\ \hline
% 0.9043 & 0.7 & 36 & huber & canberra & xyz & 10.0 \\ \hline
% 0.9093 & 0.5 & 36 & mae & euclidean & z_xy_xyz & 10.0 \\ \hline
% 0.9118 & 0.7 & 36 & mae & minkowski & z_xy_xyz & 10.0 \\ \hline
% 0.9181 & 0.3 & 36 & mae & euclidean & z_xy_xyz & 10.0 \\ \hline
% 0.9233 & 0.5 & 36 & mae & minkowski & xyz & 10.0 \\ \hline
% 0.9245 & 0.5 & 36 & mae & jaccard & xyz & 7.0 \\ \hline
% 0.9251 & 0.5 & 36 & mae & minkowski & xyz & 7.0 \\ \hline
% 0.9351 & 0.3 & 36 & huber & minkowski & z_xy_xyz & 10.0 \\ \hline
% 0.9394 & 0.7 & 36 & huber & jaccard & xyz & 10.0 \\ \hline
% 0.9408 & 0.7 & 36 & mae & canberra & abs_z_xyz & 10.0 \\ \hline
% 0.942 & 0.7 & 36 & mae & canberra & xyz & 7.0 \\ \hline
% 0.9426 & 0.3 & 36 & mse & canberra & xyz & 10.0 \\ \hline
% 0.9446 & 0.5 & 24 & mae & canberra & xyz & 7.0 \\ \hline
% 0.945 & 0.3 & 36 & mse & euclidean & z_xy_xyz & 10.0 \\ \hline
% 0.9565 & 0.7 & 36 & mae & jaccard & xyz & 10.0 \\ \hline
% 0.9672 & 0.3 & 36 & mae & canberra & xyz & 7.0 \\ \hline
% 0.972 & 0.5 & 36 & mae & jaccard & z_xy_xyz & 10.0 \\ \hline
% 0.9723 & 0.5 & 36 & mse & canberra & z_xy_xyz & 10.0 \\ \hline
% 0.9724 & 0.5 & 36 & huber & euclidean & z_xy_xyz & 10.0 \\ \hline
% 0.9773 & 0.3 & 36 & huber & canberra & xyz & 10.0 \\ \hline
% 0.9803 & 0.3 & 36 & huber & canberra & xyz & 10.0 \\ \hline
% 0.985 & 0.5 & 36 & huber & minkowski & xyz & 7.0 \\ \hline
% 0.986 & 0.3 & 36 & mae & minkowski & z_xy_xyz & 10.0 \\ \hline
% 0.9867 & 0.3 & 36 & mae & minkowski & xyz & 10.0 \\ \hline
% 0.9896 & 0.3 & 36 & mae & jaccard & xyz & 7.0 \\ \hline
% 0.9914 & 0.3 & 36 & mse & minkowski & xyz & 10.0 \\ \hline
% 0.9921 & 0.5 & 36 & mae & minkowski & xyz & 10.0 \\ \hline
% 0.9959 & 0.7 & 36 & huber & canberra & xyz & 7.0 \\ \hline
% 0.9964 & 0.3 & 36 & mse & canberra & xyz & 10.0 \\ \hline
% 1.001 & 0.3 & 36 & mae & canberra & xyz & 7.0 \\ \hline
% 1.0018 & 0.3 & 36 & mae & euclidean & xyz & 7.0 \\ \hline
% 1.0048 & 0.5 & 36 & mae & jaccard & xyz & 7.0 \\ \hline
% 1.0071 & 0.3 & 36 & mae & minkowski & z_xy_xyz & 10.0 \\ \hline
% 1.01 & 0.3 & 36 & huber & jaccard & xyz & 7.0 \\ \hline
% 1.0159 & 0.3 & 24 & mae & canberra & xyz & 10.0 \\ \hline
% 1.0165 & 0.5 & 24 & mae & canberra & z_xy_xyz & 10.0 \\ \hline
% 1.0271 & 0.5 & 36 & huber & minkowski & abs_z_xyz & 10.0 \\ \hline
% 1.0306 & 0.3 & 36 & huber & euclidean & xyz & 10.0 \\ \hline
% 1.0321 & 0.7 & 36 & mae & euclidean & z_xy_xyz & 10.0 \\ \hline
% 1.0366 & 0.3 & 36 & mae & euclidean & xyz & 10.0 \\ \hline
% 1.0382 & 0.5 & 36 & mse & euclidean & xyz & 10.0 \\ \hline


\end{tabular}
\caption{Regression model, CSL, results. (conv\_channels = [16, 24], conv\_kernels = [5, 5], activation\_func = relu)}
\label{tab:csl_regr_full_results}
\end{table}

\end{landscape}
\restoregeometry


==> tables/Tables/csl_rnn_full_results.tex <==
\newgeometry{margin=1cm} % modify this if you need even more space
\begin{landscape}

\begin{table}[h!]
\centering


\begin{tabular}{ |c|c|c|c|c|c| }
\hline
\textbf{Test error (m.)} & \textbf{metrics} & \textbf{n\_start\_points} &  \textbf{noise\_to\_first\_points} &
 \textbf{rnn\_num\_layers} &
 \textbf{teacher\_forcing} \\ \hline
0.2975 & euclidean & 20 & 1.5 & 3 & 0.2 \\ \hline
0.3202 & minkowski & 20 & 1.5 & 3 & 0.2 \\ \hline
0.3227 & euclidean & 10 & 1.5 & 2 & 0.2 \\ \hline
0.3228 & euclidean & 10 & 3.0 & 2 & 0.2 \\ \hline
0.3305 & canberra & 20 & 0.0 & 2 & 0.0 \\ \hline
0.3318 & minkowski & 20 & 3.0 & 2 & 0.2 \\ \hline
0.3338 & canberra & 10 & 0.0 & 2 & 0.0 \\ \hline
0.3365 & minkowski & 10 & 3.0 & 2 & 0.2 \\ \hline
0.3498 & minkowski & 20 & 0.0 & 2 & 0.2 \\ \hline
0.3546 & canberra & 10 & 0.0 & 2 & 0.2 \\ \hline
0.361 & minkowski & 20 & 3.0 & 3 & 0.0 \\ \hline
0.3682 & canberra & 20 & 1.5 & 2 & 0.0 \\ \hline
0.3684 & euclidean & 10 & 0.0 & 2 & 0.0 \\ \hline
0.3723 & canberra & 20 & 3.0 & 3 & 0.0 \\ \hline
0.3795 & euclidean & 10 & 3.0 & 3 & 0.0 \\ \hline
0.3821 & canberra & 10 & 1.5 & 3 & 0.0 \\ \hline
0.3826 & euclidean & 20 & 3.0 & 2 & 0.2 \\ \hline
0.3833 & canberra & 10 & 1.5 & 3 & 0.2 \\ \hline
0.3893 & canberra & 10 & 3.0 & 2 & 0.2 \\ \hline
0.3963 & canberra & 10 & 0.0 & 3 & 0.2 \\ \hline
0.401 & euclidean & 20 & 0.0 & 2 & 0.2 \\ \hline
0.4059 & canberra & 10 & 3.0 & 3 & 0.2 \\ \hline
0.4061 & euclidean & 10 & 1.5 & 2 & 0.0 \\ \hline
0.4222 & canberra & 10 & 1.5 & 2 & 0.0 \\ \hline
0.427 & canberra & 20 & 0.0 & 3 & 0.0 \\ \hline
0.4357 & canberra & 20 & 1.5 & 3 & 0.0 \\ \hline
0.4398 & canberra & 10 & 3.0 & 2 & 0.0 \\ \hline
0.441 & euclidean & 20 & 1.5 & 3 & 0.0 \\ \hline
0.4413 & euclidean & 20 & 3.0 & 3 & 0.0 \\ \hline
0.4548 & canberra & 10 & 1.5 & 2 & 0.2 \\ \hline
0.4661 & canberra & 20 & 1.5 & 3 & 0.2 \\ \hline
0.4673 & canberra & 10 & 0.0 & 3 & 0.0 \\ \hline
0.468 & minkowski & 10 & 0.0 & 3 & 0.2 \\ \hline
0.4737 & minkowski & 20 & 0.0 & 3 & 0.0 \\ \hline
0.4878 & minkowski & 10 & 0.0 & 3 & 0.0 \\ \hline
0.4972 & canberra & 20 & 3.0 & 2 & 0.0 \\ \hline
0.5084 & canberra & 10 & 3.0 & 3 & 0.0 \\ \hline
% 0.511 & minkowski & 20 & 1.5 & 3 & 0.0 \\ \hline
% 0.5364 & canberra & 20 & 0.0 & 2 & 0.2 \\ \hline
% 0.6011 & minkowski & 10 & 3.0 & 3 & 0.2 \\ \hline
% 0.6076 & canberra & 20 & 1.5 & 2 & 0.2 \\ \hline
% 0.6077 & minkowski & 10 & 1.5 & 2 & 0.2 \\ \hline
% 0.6082 & euclidean & 20 & 0.0 & 3 & 0.2 \\ \hline
% 0.6448 & minkowski & 10 & 0.0 & 2 & 0.0 \\ \hline
% 0.6801 & euclidean & 20 & 3.0 & 3 & 0.2 \\ \hline
% 0.6944 & minkowski & 10 & 1.5 & 3 & 0.0 \\ \hline
% 0.7104 & euclidean & 20 & 0.0 & 2 & 0.0 \\ \hline
% 0.7297 & minkowski & 10 & 3.0 & 2 & 0.0 \\ \hline
% 0.7398 & canberra & 20 & 3.0 & 2 & 0.2 \\ \hline
% 0.7542 & minkowski & 20 & 0.0 & 2 & 0.0 \\ \hline
% 0.7561 & minkowski & 20 & 1.5 & 2 & 0.0 \\ \hline
% 0.8011 & euclidean & 20 & 0.0 & 3 & 0.0 \\ \hline
% 0.8188 & euclidean & 10 & 3.0 & 2 & 0.0 \\ \hline
% 0.822 & euclidean & 10 & 1.5 & 3 & 0.0 \\ \hline
% 0.8488 & minkowski & 20 & 3.0 & 2 & 0.0 \\ \hline
% 0.8894 & minkowski & 10 & 1.5 & 2 & 0.0 \\ \hline
% 1.0539 & euclidean & 10 & 3.0 & 3 & 0.2 \\ \hline
% 1.0728 & euclidean & 10 & 0.0 & 2 & 0.2 \\ \hline
% 1.0923 & minkowski & 10 & 3.0 & 3 & 0.0 \\ \hline
% 1.0951 & euclidean & 20 & 1.5 & 2 & 0.2 \\ \hline
% 1.1818 & minkowski & 10 & 1.5 & 3 & 0.2 \\ \hline
% 1.2425 & minkowski & 20 & 1.5 & 2 & 0.2 \\ \hline
% 1.2483 & minkowski & 20 & 0.0 & 3 & 0.2 \\ \hline
% 1.3569 & canberra & 20 & 3.0 & 3 & 0.2 \\ \hline
% 1.427 & canberra & 20 & 0.0 & 3 & 0.2 \\ \hline
% 1.5167 & euclidean & 20 & 3.0 & 2 & 0.0 \\ \hline
% 1.5501 & euclidean & 10 & 0.0 & 3 & 0.0 \\ \hline
% 1.6474 & euclidean & 20 & 1.5 & 2 & 0.0 \\ \hline
% 2.2126 & minkowski & 10 & 0.0 & 2 & 0.2 \\ \hline
% 3.2089 & euclidean & 10 & 0.0 & 3 & 0.2 \\ \hline
% 3.9296 & minkowski & 20 & 3.0 & 3 & 0.2 \\ \hline
% 4.8224 & euclidean & 10 & 1.5 & 3 & 0.2 \\ \hline

\end{tabular}
\caption{RNN model, CSL, results. (hidden\_size = 300, image\_size = 24, loss = mse, mag\_comp = xyz, step = 0.5 s, window = 7 s)}
\label{tab:csl_rnn_full_results}
\end{table}

\end{landscape}
\restoregeometry


==> tables/Tables/loomis_regr_full_results.tex <==
\newgeometry{margin=1cm} % modify this if you need even more space
\begin{landscape}

\begin{table}[h!]
\centering


\begin{tabular}{ |c|c|c|c|c|c|c| }
\hline
\textbf{Test error (m.)} & \textbf{dropout} & \textbf{image\_size} &  \textbf{loss} &
 \textbf{metrics} &
 \textbf{mag\_comp} &
 \textbf{window}
 \\ \hline
3.9967 & 0.3 & 36 & huber & canberra & z\_xy\_xyz & 10.0 \\ \hline
4.3771 & 0.7 & 36 & mae & euclidean & abs\_z\_xyz & 10.0 \\ \hline
4.5144 & 0.7 & 36 & huber & minkowski & z\_xy\_xyz & 10.0 \\ \hline
4.552 & 0.5 & 36 & huber & minkowski & z\_xy\_xyz & 10.0 \\ \hline
4.6317 & 0.5 & 36 & huber & jaccard & abs\_z\_xyz & 10.0 \\ \hline
4.6542 & 0.3 & 36 & mae & jaccard & z\_xy\_xyz & 10.0 \\ \hline
4.6557 & 0.7 & 36 & mse & canberra & abs\_z\_xyz & 10.0 \\ \hline
4.6961 & 0.7 & 36 & mae & euclidean & abs\_z\_xyz & 10.0 \\ \hline
4.7049 & 0.3 & 36 & mse & canberra & abs\_z\_xyz & 10.0 \\ \hline
4.7104 & 0.7 & 36 & mae & euclidean & z\_xy\_xyz & 10.0 \\ \hline
4.724 & 0.5 & 36 & mse & minkowski & xyz & 10.0 \\ \hline
4.7478 & 0.7 & 36 & huber & canberra & z\_xy\_xyz & 10.0 \\ \hline
4.7594 & 0.7 & 36 & huber & minkowski & xyz & 10.0 \\ \hline
4.7632 & 0.5 & 36 & mae & minkowski & z\_xy\_xyz & 10.0 \\ \hline
4.7677 & 0.7 & 36 & mae & canberra & abs\_z\_xyz & 10.0 \\ \hline
4.7694 & 0.7 & 36 & mae & euclidean & xyz & 10.0 \\ \hline
4.7747 & 0.3 & 36 & huber & canberra & abs\_z\_xyz & 10.0 \\ \hline
4.7833 & 0.3 & 36 & mae & euclidean & z\_xy\_xyz & 10.0 \\ \hline
4.7906 & 0.5 & 36 & mae & euclidean & xyz & 10.0 \\ \hline
4.7932 & 0.7 & 36 & mse & minkowski & z\_xy\_xyz & 10.0 \\ \hline
4.8096 & 0.5 & 36 & mae & euclidean & abs\_z\_xyz & 10.0 \\ \hline
4.8149 & 0.7 & 36 & huber & canberra & xyz & 10.0 \\ \hline
4.8379 & 0.3 & 36 & mse & minkowski & z\_xy\_xyz & 10.0 \\ \hline
4.8385 & 0.5 & 36 & mae & euclidean & z\_xy\_xyz & 10.0 \\ \hline
4.8585 & 0.5 & 36 & huber & euclidean & z\_xy\_xyz & 10.0 \\ \hline
4.8609 & 0.5 & 36 & huber & canberra & abs\_z\_xyz & 10.0 \\ \hline
4.8705 & 0.3 & 36 & mae & minkowski & z\_xy\_xyz & 10.0 \\ \hline
4.8862 & 0.5 & 36 & mse & canberra & z\_xy\_xyz & 10.0 \\ \hline
4.8894 & 0.7 & 36 & mse & minkowski & abs\_z\_xyz & 10.0 \\ \hline
4.8934 & 0.7 & 36 & mae & minkowski & xyz & 10.0 \\ \hline
4.896 & 0.3 & 36 & mae & jaccard & abs\_z\_xyz & 10.0 \\ \hline
4.8998 & 0.3 & 24 & mse & canberra & z\_xy\_xyz & 10.0 \\ \hline
4.9154 & 0.5 & 36 & huber & jaccard & abs\_z\_xyz & 10.0 \\ \hline
4.9164 & 0.7 & 36 & huber & minkowski & abs\_z\_xyz & 10.0 \\ \hline
4.9237 & 0.7 & 36 & mse & jaccard & z\_xy\_xyz & 10.0 \\ \hline
4.9247 & 0.7 & 36 & mse & canberra & z\_xy\_xyz & 10.0 \\ \hline
4.9378 & 0.3 & 36 & mae & canberra & z\_xy\_xyz & 10.0 \\ \hline
% 4.953 & 0.5 & 36 & mae & minkowski & z\_xy\_xyz & 10.0 \\ \hline
% 4.9661 & 0.5 & 36 & mae & canberra & abs\_z\_xyz & 10.0 \\ \hline
% 4.9757 & 0.3 & 24 & mae & euclidean & z\_xy\_xyz & 10.0 \\ \hline
% 4.9885 & 0.5 & 36 & mae & minkowski & xyz & 10.0 \\ \hline
% 4.9954 & 0.5 & 36 & mae & canberra & xyz & 10.0 \\ \hline
% 5.0145 & 0.5 & 36 & mse & minkowski & z\_xy\_xyz & 10.0 \\ \hline
% 5.0153 & 0.3 & 36 & mae & euclidean & abs\_z\_xyz & 10.0 \\ \hline
% 5.0301 & 0.5 & 36 & mse & canberra & abs\_z\_xyz & 10.0 \\ \hline
% 5.0362 & 0.7 & 36 & mse & canberra & abs\_z\_xyz & 10.0 \\ \hline
% 5.052 & 0.3 & 36 & huber & euclidean & z\_xy\_xyz & 10.0 \\ \hline
% 5.0548 & 0.3 & 24 & mse & canberra & abs\_z\_xyz & 10.0 \\ \hline
% 5.0846 & 0.5 & 36 & mae & euclidean & abs\_z\_xyz & 10.0 \\ \hline
% 5.0896 & 0.7 & 36 & huber & jaccard & z\_xy\_xyz & 10.0 \\ \hline


\end{tabular}
\caption{Regression model, Loomis, results. (conv\_channels = [16, 24], conv\_kernels = [5, 5], activation\_func = relu)}
\label{tab:loomis_regr_full_results}
\end{table}

\end{landscape}
\restoregeometry


==> tables/Tables/loomis_rnn_full_results.tex <==
\newgeometry{margin=1cm} % modify this if you need even more space
\begin{landscape}

\begin{table}[h!]
\centering


\begin{tabular}{ |c|c|c|c|c|c| }
\hline
\textbf{Test error (m.)} & \textbf{metrics} & \textbf{n\_start\_points} &  \textbf{noise\_to\_first\_points} &
 \textbf{rnn\_num\_layers} &
 \textbf{teacher\_forcing} \\ \hline
1.0519 & canberra & 10 & 0.0 & 2 & 0.1 \\ \hline
1.1142 & canberra & 10 & 1.5 & 2 & 0.1 \\ \hline
1.1306 & canberra & 10 & 0.0 & 3 & 0.2 \\ \hline
1.2331 & canberra & 10 & 3.0 & 2 & 0.2 \\ \hline
1.2461 & canberra & 10 & 3.0 & 3 & 0.1 \\ \hline
1.2515 & canberra & 10 & 1.5 & 3 & 0.2 \\ \hline
1.2714 & euclidean & 10 & 3.0 & 2 & 0.2 \\ \hline
1.2786 & canberra & 10 & 3.0 & 2 & 0.1 \\ \hline
1.2973 & canberra & 10 & 1.5 & 2 & 0.2 \\ \hline
1.3236 & canberra & 10 & 1.5 & 3 & 0.1 \\ \hline
1.3328 & canberra & 20 & 0.0 & 2 & 0.1 \\ \hline
1.3943 & canberra & 10 & 0.0 & 2 & 0.2 \\ \hline
1.4016 & canberra & 10 & 3.0 & 3 & 0.2 \\ \hline
1.4073 & canberra & 10 & 0.0 & 3 & 0.1 \\ \hline
1.4541 & canberra & 20 & 1.5 & 2 & 0.2 \\ \hline
1.482 & minkowski & 10 & 3.0 & 2 & 0.1 \\ \hline
1.4865 & minkowski & 10 & 1.5 & 2 & 0.2 \\ \hline
1.5205 & minkowski & 20 & 0.0 & 2 & 0.2 \\ \hline
1.5257 & minkowski & 10 & 3.0 & 2 & 0.2 \\ \hline
1.5675 & euclidean & 10 & 0.0 & 2 & 0.2 \\ \hline
1.6008 & euclidean & 10 & 3.0 & 2 & 0.1 \\ \hline
1.6386 & canberra & 20 & 0.0 & 3 & 0.1 \\ \hline
1.6504 & euclidean & 10 & 1.5 & 2 & 0.1 \\ \hline
1.6804 & canberra & 20 & 3.0 & 3 & 0.1 \\ \hline
1.6911 & minkowski & 10 & 0.0 & 2 & 0.2 \\ \hline
1.7172 & minkowski & 10 & 0.0 & 2 & 0.1 \\ \hline
1.7704 & euclidean & 10 & 0.0 & 2 & 0.1 \\ \hline
1.7827 & canberra & 20 & 0.0 & 3 & 0.2 \\ \hline
1.8212 & euclidean & 10 & 3.0 & 3 & 0.1 \\ \hline
1.8279 & euclidean & 20 & 1.5 & 2 & 0.2 \\ \hline
1.8781 & canberra & 20 & 3.0 & 2 & 0.2 \\ \hline
1.886 & canberra & 20 & 1.5 & 2 & 0.1 \\ \hline
1.927 & canberra & 20 & 3.0 & 2 & 0.1 \\ \hline
2.0244 & canberra & 20 & 1.5 & 3 & 0.1 \\ \hline
2.0674 & euclidean & 10 & 1.5 & 2 & 0.2 \\ \hline
2.1253 & euclidean & 10 & 1.5 & 3 & 0.2 \\ \hline
2.2143 & minkowski & 10 & 0.0 & 3 & 0.2 \\ \hline
2.2714 & canberra & 20 & 1.5 & 3 & 0.2 \\ \hline
% 2.3546 & minkowski & 20 & 0.0 & 2 & 0.1 \\ \hline
% 2.4516 & minkowski & 10 & 3.0 & 3 & 0.1 \\ \hline
% 2.4635 & euclidean & 20 & 0.0 & 2 & 0.1 \\ \hline
% 2.5384 & euclidean & 20 & 0.0 & 2 & 0.2 \\ \hline
% 2.5548 & canberra & 20 & 3.0 & 3 & 0.2 \\ \hline
% 2.5719 & minkowski & 10 & 3.0 & 3 & 0.2 \\ \hline
% 2.7047 & euclidean & 20 & 0.0 & 3 & 0.1 \\ \hline
% 2.7112 & minkowski & 20 & 3.0 & 2 & 0.1 \\ \hline
% 2.7423 & euclidean & 20 & 3.0 & 3 & 0.2 \\ \hline
% 2.7626 & euclidean & 10 & 1.5 & 3 & 0.1 \\ \hline
% 2.8195 & euclidean & 20 & 0.0 & 3 & 0.2 \\ \hline
% 2.8329 & minkowski & 20 & 1.5 & 3 & 0.1 \\ \hline
% 2.8688 & minkowski & 20 & 1.5 & 3 & 0.2 \\ \hline
% 2.8782 & euclidean & 20 & 3.0 & 2 & 0.1 \\ \hline
% 2.9294 & euclidean & 20 & 1.5 & 3 & 0.1 \\ \hline
% 2.977 & minkowski & 20 & 3.0 & 3 & 0.2 \\ \hline
% 3.002 & minkowski & 20 & 3.0 & 3 & 0.1 \\ \hline
% 3.1532 & minkowski & 10 & 1.5 & 3 & 0.1 \\ \hline
% 3.1547 & minkowski & 10 & 1.5 & 2 & 0.1 \\ \hline
% 3.1679 & euclidean & 10 & 3.0 & 3 & 0.2 \\ \hline
% 3.2346 & canberra & 20 & 0.0 & 2 & 0.2 \\ \hline
% 3.2918 & minkowski & 20 & 0.0 & 3 & 0.2 \\ \hline
% 3.3681 & minkowski & 10 & 1.5 & 3 & 0.2 \\ \hline
% 3.52 & euclidean & 20 & 3.0 & 2 & 0.2 \\ \hline
% 3.5729 & euclidean & 10 & 0.0 & 3 & 0.1 \\ \hline
% 3.6353 & minkowski & 20 & 0.0 & 3 & 0.1 \\ \hline
% 3.6952 & euclidean & 10 & 0.0 & 3 & 0.2 \\ \hline
% 3.7674 & minkowski & 20 & 1.5 & 2 & 0.1 \\ \hline
% 3.7799 & minkowski & 10 & 0.0 & 3 & 0.1 \\ \hline
% 4.1494 & minkowski & 20 & 3.0 & 2 & 0.2 \\ \hline
% 4.472 & minkowski & 20 & 1.5 & 2 & 0.2 \\ \hline
% 4.4773 & euclidean & 20 & 1.5 & 3 & 0.2 \\ \hline
% 4.9335 & euclidean & 20 & 3.0 & 3 & 0.1 \\ \hline
% 7.021 & euclidean & 20 & 1.5 & 2 & 0.1 \\ \hline

\end{tabular}
\caption{RNN model, Loomis, results. (hidden\_size = 300, image\_size = 24, loss = mse, mag\_comp = xyz, step = 0.5 s, window = 7 s)}
\label{tab:loomis_rnn_full_results}
\end{table}

\end{landscape}
\restoregeometry


==> tables/Tables/meta_classifier_results.tex <==
\begin{table}[h!]
\centering

\begin{tabular}{ |c|c|c| }
\hline
\textbf{Building} & \textbf{Meta-classifier test error (m)} & \textbf{Meta-classifier accuracy (\%)} \\ \hline
CSL & 0.95 & 55.74 \\ \hline
Loomis & 4.62 & 51.04 \\ \hline
Talbot & 4.49 & 47.95  \\ \hline

\end{tabular}
\caption{Ensembling results}
\label{tab:ensembling_results}
\end{table}


==> tables/Tables/multi_task_results.tex <==
\begin{table}[h!]
\centering

\begin{tabular}{ |c|c|c| }
\hline
\textbf{Building} & \textbf{Test error (m)} & \textbf{Accuracy (\%)} \\ \hline
CSL & 1.27 & 93.38 \\ \hline
Loomis & 5.15 & 72.89 \\ \hline
Talbot & 6.04 & 70.37  \\ \hline

\end{tabular}
\caption{Multi-task results}
\label{tab:multi_task_results}
\end{table}

==> tables/Tables/regression_results.tex <==
\begin{table}[h!]
\centering

\begin{tabular}{ |c|c|c| }
\hline
\textbf{Building} & \textbf{Test error (m)} \\ \hline
CSL & 0.58 \\ \hline
Loomis & 4.00 \\ \hline
Talbot & 3.90  \\ \hline

\end{tabular}
\caption{Regression model results}
\label{tab:regr_results}
\end{table}

==> tables/Tables/rnn_results.tex <==
\begin{table}[h!]
\centering

\begin{tabular}{ |c|c|c| }
\hline
\textbf{Building} & \textbf{Test error (m)} \\ \hline
CSL & 0.30 \\ \hline
Loomis & 1.05 \\ \hline
Talbot & 0.89 \\ \hline

\end{tabular}
\caption{RNN model results}
\label{tab:rnn_results}
\end{table}

==> tables/Tables/talbot_regr_full_results.tex <==
\newgeometry{margin=1cm} % modify this if you need even more space
\begin{landscape}

\begin{table}[h!]
\centering


\begin{tabular}{ |c|c|c|c|c|c|c| }
\hline
\textbf{Test error (m.)} & \textbf{dropout} & \textbf{image\_size} &  \textbf{loss} &
 \textbf{metrics} &
 \textbf{mag\_comp} &
 \textbf{window}
 \\ \hline
3.8988 & 0.5 & 36 & mae & canberra & xyz & 10.0 \\ \hline
4.0127 & 0.3 & 36 & mae & canberra & xyz & 10.0 \\ \hline
4.0314 & 0.7 & 36 & mse & euclidean & xyz & 10.0 \\ \hline
4.042 & 0.5 & 36 & mae & canberra & xyz & 7.0 \\ \hline
4.0807 & 0.5 & 36 & huber & canberra & xyz & 10.0 \\ \hline
4.0932 & 0.7 & 36 & mae & minkowski & xyz & 7.0 \\ \hline
4.1043 & 0.5 & 36 & mae & jaccard & xyz & 10.0 \\ \hline
4.1266 & 0.7 & 36 & mae & canberra & xyz & 7.0 \\ \hline
4.142 & 0.3 & 36 & huber & canberra & xyz & 10.0 \\ \hline
4.1738 & 0.7 & 36 & mse & canberra & xyz & 10.0 \\ \hline
4.1743 & 0.5 & 36 & mse & canberra & xyz & 10.0 \\ \hline
4.1888 & 0.3 & 24 & mae & canberra & xyz & 7.0 \\ \hline
4.2031 & 0.5 & 36 & mse & canberra & xyz & 10.0 \\ \hline
4.2187 & 0.7 & 36 & mae & euclidean & xyz & 7.0 \\ \hline
4.2266 & 0.7 & 36 & mae & jaccard & xyz & 10.0 \\ \hline
4.2294 & 0.5 & 36 & mae & jaccard & xyz & 7.0 \\ \hline
4.2621 & 0.5 & 36 & mae & canberra & xyz & 10.0 \\ \hline
4.271 & 0.5 & 36 & huber & minkowski & xyz & 10.0 \\ \hline
4.2758 & 0.7 & 36 & mae & jaccard & xyz & 10.0 \\ \hline
4.2829 & 0.3 & 36 & huber & canberra & xyz & 10.0 \\ \hline
4.2916 & 0.7 & 36 & mae & canberra & xyz & 7.0 \\ \hline
4.2963 & 0.3 & 36 & huber & canberra & xyz & 7.0 \\ \hline
4.3073 & 0.7 & 36 & huber & canberra & xyz & 10.0 \\ \hline
4.3116 & 0.5 & 36 & mae & minkowski & xyz & 7.0 \\ \hline
4.312 & 0.5 & 36 & mse & canberra & xyz & 10.0 \\ \hline
4.3153 & 0.5 & 36 & huber & canberra & xyz & 10.0 \\ \hline
4.3212 & 0.3 & 36 & mse & jaccard & xyz & 10.0 \\ \hline
4.3287 & 0.7 & 36 & mae & canberra & xyz & 10.0 \\ \hline
4.3314 & 0.3 & 36 & mse & canberra & xyz & 10.0 \\ \hline
4.3527 & 0.3 & 36 & mae & canberra & xyz & 7.0 \\ \hline
4.3659 & 0.5 & 36 & huber & canberra & xyz & 10.0 \\ \hline
4.3885 & 0.7 & 36 & mse & canberra & xyz & 10.0 \\ \hline
4.4312 & 0.3 & 36 & mae & minkowski & xyz & 7.0 \\ \hline
4.434 & 0.3 & 36 & huber & euclidean & xyz & 10.0 \\ \hline
4.4444 & 0.3 & 36 & mae & euclidean & xyz & 7.0 \\ \hline
4.4458 & 0.7 & 36 & huber & canberra & xyz & 10.0 \\ \hline
4.4595 & 0.5 & 36 & mae & euclidean & xyz & 10.0 \\ \hline
% 4.4673 & 0.5 & 36 & mse & jaccard & xyz & 10.0 \\ \hline
% 4.4694 & 0.5 & 36 & mse & canberra & xyz & 7.0 \\ \hline
% 4.4721 & 0.5 & 36 & mse & jaccard & xyz & 10.0 \\ \hline
% 4.4854 & 0.5 & 36 & mae & euclidean & xyz & 10.0 \\ \hline
% 4.4955 & 0.3 & 36 & mse & canberra & xyz & 10.0 \\ \hline
% 4.4965 & 0.3 & 36 & mse & minkowski & xyz & 7.0 \\ \hline
% 4.5215 & 0.5 & 36 & huber & jaccard & xyz & 7.0 \\ \hline
% 4.5231 & 0.7 & 36 & mse & euclidean & xyz & 10.0 \\ \hline
% 4.5301 & 0.7 & 36 & huber & canberra & xyz & 7.0 \\ \hline
% 4.5303 & 0.3 & 24 & huber & minkowski & xyz & 10.0 \\ \hline
% 4.5349 & 0.3 & 24 & mse & canberra & xyz & 10.0 \\ \hline
% 4.5372 & 0.7 & 36 & mse & canberra & xyz & 10.0 \\ \hline
% 4.5458 & 0.7 & 36 & mae & canberra & xyz & 10.0 \\ \hline


\end{tabular}
\caption{Regression model, Talbot, results. (conv\_channels = [16, 24], conv\_kernels = [5, 5], activation\_func = relu)}
\label{tab:talbot_regr_full_results}
\end{table}

\end{landscape}
\restoregeometry


==> tables/Tables/talbot_rnn_full_results.tex <==
\newgeometry{margin=1cm} % modify this if you need even more space
\begin{landscape}

\begin{table}[h!]
\centering


\begin{tabular}{ |c|c|c|c|c|c| }
\hline
\textbf{Test error (m.)} & \textbf{metrics} & \textbf{n\_start\_points} &  \textbf{noise\_to\_first\_points} &
 \textbf{rnn\_num\_layers} &
 \textbf{teacher\_forcing} \\ \hline
0.8862 & canberra & 10 & 3.0 & 2 & 0.2 \\ \hline
0.9787 & canberra & 10 & 1.5 & 3 & 0.2 \\ \hline
1.0232 & canberra & 10 & 1.5 & 2 & 0.2 \\ \hline
1.0365 & canberra & 10 & 0.0 & 3 & 0.2 \\ \hline
1.0452 & canberra & 10 & 0.0 & 2 & 0.2 \\ \hline
1.1186 & canberra & 10 & 3.0 & 2 & 0.1 \\ \hline
1.1504 & canberra & 10 & 1.5 & 2 & 0.1 \\ \hline
1.2564 & canberra & 10 & 0.0 & 2 & 0.1 \\ \hline
1.2856 & canberra & 20 & 1.5 & 2 & 0.1 \\ \hline
1.3397 & minkowski & 20 & 3.0 & 3 & 0.1 \\ \hline
1.4206 & euclidean & 10 & 1.5 & 3 & 0.1 \\ \hline
1.4615 & canberra & 20 & 0.0 & 2 & 0.1 \\ \hline
1.5168 & canberra & 20 & 3.0 & 3 & 0.2 \\ \hline
1.5176 & canberra & 10 & 0.0 & 3 & 0.1 \\ \hline
1.5292 & canberra & 10 & 1.5 & 3 & 0.1 \\ \hline
1.5514 & canberra & 20 & 3.0 & 2 & 0.1 \\ \hline
1.5544 & canberra & 20 & 0.0 & 3 & 0.2 \\ \hline
1.5823 & euclidean & 10 & 3.0 & 3 & 0.2 \\ \hline
1.5853 & euclidean & 10 & 1.5 & 2 & 0.1 \\ \hline
1.6394 & minkowski & 10 & 3.0 & 2 & 0.1 \\ \hline
1.6751 & canberra & 20 & 1.5 & 3 & 0.1 \\ \hline
1.6758 & minkowski & 10 & 1.5 & 3 & 0.2 \\ \hline
1.6768 & canberra & 10 & 3.0 & 3 & 0.1 \\ \hline
1.6943 & euclidean & 10 & 1.5 & 2 & 0.2 \\ \hline
1.7139 & euclidean & 10 & 0.0 & 2 & 0.1 \\ \hline
1.718 & euclidean & 20 & 0.0 & 2 & 0.1 \\ \hline
1.764 & minkowski & 20 & 0.0 & 3 & 0.1 \\ \hline
1.7768 & euclidean & 10 & 3.0 & 3 & 0.1 \\ \hline
1.9351 & minkowski & 10 & 1.5 & 2 & 0.1 \\ \hline
1.9769 & euclidean & 20 & 1.5 & 3 & 0.2 \\ \hline
1.9892 & canberra & 20 & 1.5 & 2 & 0.2 \\ \hline
2.047 & canberra & 20 & 0.0 & 2 & 0.2 \\ \hline
2.1131 & canberra & 20 & 3.0 & 2 & 0.2 \\ \hline
2.1517 & minkowski & 10 & 3.0 & 3 & 0.1 \\ \hline
2.1618 & minkowski & 10 & 0.0 & 3 & 0.2 \\ \hline
2.2318 & canberra & 20 & 0.0 & 3 & 0.1 \\ \hline
2.311 & minkowski & 10 & 0.0 & 2 & 0.2 \\ \hline
% 2.7397 & canberra & 20 & 1.5 & 3 & 0.2 \\ \hline
% 2.9599 & canberra & 10 & 3.0 & 3 & 0.2 \\ \hline
% 3.1472 & euclidean & 20 & 0.0 & 3 & 0.2 \\ \hline
% 3.3881 & euclidean & 20 & 3.0 & 2 & 0.1 \\ \hline
% 3.4803 & minkowski & 10 & 1.5 & 3 & 0.1 \\ \hline
% 3.5129 & minkowski & 10 & 1.5 & 2 & 0.2 \\ \hline
% 3.5224 & minkowski & 20 & 1.5 & 3 & 0.2 \\ \hline
% 3.5562 & euclidean & 10 & 3.0 & 2 & 0.1 \\ \hline
% 3.577 & euclidean & 20 & 1.5 & 2 & 0.1 \\ \hline
% 3.5821 & euclidean & 20 & 3.0 & 3 & 0.1 \\ \hline
% 3.5979 & minkowski & 20 & 3.0 & 2 & 0.1 \\ \hline
% 3.6073 & euclidean & 20 & 0.0 & 3 & 0.1 \\ \hline
% 3.6118 & minkowski & 10 & 0.0 & 3 & 0.1 \\ \hline
% 3.6277 & minkowski & 10 & 3.0 & 3 & 0.2 \\ \hline
% 3.6763 & euclidean & 10 & 1.5 & 3 & 0.2 \\ \hline
% 3.6767 & minkowski & 10 & 0.0 & 2 & 0.1 \\ \hline
% 3.6926 & minkowski & 20 & 0.0 & 2 & 0.1 \\ \hline
% 3.7298 & minkowski & 10 & 3.0 & 2 & 0.2 \\ \hline
% 3.7996 & minkowski & 20 & 0.0 & 3 & 0.2 \\ \hline
% 3.8431 & euclidean & 10 & 3.0 & 2 & 0.2 \\ \hline
% 3.8509 & euclidean & 10 & 0.0 & 2 & 0.2 \\ \hline
% 3.9195 & minkowski & 20 & 3.0 & 3 & 0.2 \\ \hline
% 3.9261 & minkowski & 20 & 1.5 & 2 & 0.2 \\ \hline
% 3.9569 & canberra & 20 & 3.0 & 3 & 0.1 \\ \hline
% 4.2663 & minkowski & 20 & 1.5 & 2 & 0.1 \\ \hline
% 4.2669 & euclidean & 10 & 0.0 & 3 & 0.2 \\ \hline
% 4.3461 & minkowski & 20 & 0.0 & 2 & 0.2 \\ \hline
% 4.35 & euclidean & 20 & 0.0 & 2 & 0.2 \\ \hline
% 4.3912 & euclidean & 10 & 0.0 & 3 & 0.1 \\ \hline
% 4.3998 & euclidean & 20 & 1.5 & 3 & 0.1 \\ \hline
% 4.4739 & minkowski & 20 & 1.5 & 3 & 0.1 \\ \hline
% 4.543 & minkowski & 20 & 3.0 & 2 & 0.2 \\ \hline
% 4.6651 & euclidean & 20 & 3.0 & 3 & 0.2 \\ \hline
% 5.006 & euclidean & 20 & 3.0 & 2 & 0.2 \\ \hline
% 5.1041 & euclidean & 20 & 1.5 & 2 & 0.2 \\ \hline

\end{tabular}
\caption{RNN model, Talbot, results. (hidden\_size = 300, image\_size = 24, loss = mse, mag\_comp = xyz, step = 0.5 s, window = 7 s)}
\label{tab:talbot_rnn_full_results}
\end{table}

\end{landscape}
\restoregeometry

